Practical Attacks Against Privacy and Availability in 4G/LTE Mobile Communication Systems

Mobile communication systems now constitute an essential part of life throughout the world. Fourth generation "Long Term Evolution" (LTE) mobile communication networks are being deployed. The LTE suite of specifications is considered to be significantly better than its predecessors not only in terms of functionality but also with respect to security and privacy for subscribers. We carefully analyzed LTE access network protocol specifications and uncovered several vulnerabilities. Using commercial LTE mobile devices in real LTE networks, we demonstrate inexpensive, and practical attacks exploiting these vulnerabilities. Our first class of attacks consists of three different ways of making an LTE device leak its location: A semi-passive attacker can locate an LTE device within a 2 sq.km area within a city whereas an active attacker can precisely locate an LTE device using GPS co-ordinates or trilateration via cell-tower signal strength information. Our second class of attacks can persistently deny some or all services to a target LTE device. To the best of our knowledge, our work constitutes the first publicly reported practical attacks against LTE access network protocols. We present several countermeasures to resist our specific attacks. We also discuss possible trade-offs that may explain why these vulnerabilities exist and recommend that safety margins introduced into future specifications to address such trade-offs should incorporate greater agility to accommodate subsequent changes in the trade-off equilibrium.

==> full-version.tex <==

% ---------------------------------------------
% This is the full version
% ---------------------------------------------



% ---------------------------------------------
% This is the submission version
% ---------------------------------------------
%\def\issubmission{1}  
%\def\isanonymous{1}  
%\def\iscomments{1}
%\def\ismodel{1}
%\def\isshaphered{1}
\def\isfullversion{1} 
\input{main}
% We leave out the model for now


%\def\isfullversion{1}  
%\def\isanonymous{1}  
%\input{shepherd.tex}


